Improving Pseudo-Time Stepping Convergence for CFD Simulations With Neural Networks

Computational fluid dynamics (CFD) simulations of viscous fluids described by the Navier-Stokes equations are considered. Depending on the Reynolds number of the flow, the Navier-Stokes equations may exhibit a highly nonlinear behavior. The system of nonlinear equations resulting from the discretization of the Navier-Stokes equations can be solved using nonlinear iteration methods, such as Newton's method. However, fast quadratic convergence is typically only obtained in a local neighborhood of the solution, and for many configurations, the classical Newton iteration does not converge at all. In such cases, so-called globalization techniques may help to improve convergence. In this paper, pseudo-transient continuation is employed in order to improve nonlinear convergence. The classical algorithm is enhanced by a neural network model that is trained to predict a local pseudo-time step. Generalization of the novel approach is facilitated by predicting the local pseudo-time step separately on each element using only local information on a patch of adjacent elements as input. Numerical results for standard benchmark problems, including flow through a backward facing step geometry and Couette flow, show the performance of the machine learning-enhanced globalization approach; as the software for the simulations, the CFD module of COMSOL Multiphysics is employed.

==> Figures/Newton+CFL/B1.tex <==

\begin{tikzpicture}[scale=0.8]
\begin{axis}[
    title = B1,
    legend pos = north west,
    xlabel={Simulation number},
    ylabel={Required number of iterations}
    ]
    \addplot [
        scatter,
        only marks,
        point meta=explicit symbolic,
        scatter/classes={
            a={mark=*,black},
            b={mark=triangle*,black!50},
            c={mark=triangle*,black!20},
            d={mark=pentagon*,black!50},
            e={mark=pentagon*,black!20}% <-- don't add comma
        },
    ] table [meta=label] {
        x      y        label
        1 6 d
2 6 d
3 6 d
4 6 d
5 17 d
6 19 d
7 24 d
8 26 d
9 31 d
10 33 d
11 34 d
12 37 d
13 40 d
14 48 d
15 61 d
16 64 d
17 82 d
18 100 d
19 100 d
20 100 d
21 100 d
22 100 d
23 100 d
24 100 d
1 7 e
2 7 e
3 7 e
4 7 e
5 17 e
6 17 e
7 20 e
8 21 e
9 27 e
10 33 e
11 38 e
12 50 e
13 51 e
14 53 e
15 65 e
16 66 e
17 87 e
18 92 e
19 100 e
20 100 e
21 100 e
22 100 e
23 100 e
24 100 e
1 7 b
2 8 b
3 9 b
4 11 b
5 28 b
6 30 b
7 46 b
8 51 b
9 51 b
10 54 b
11 65 b
12 75 b
13 75 b
14 81 b
15 91 b
16 93 b
17 100 b
18 100 b
19 100 b
20 100 b
21 100 b
22 100 b
23 100 b
24 100 b
1 6 c
2 6 c
3 6 c
4 6 c
5 17 c
6 19 c
7 24 c
8 26 c
9 31 c
10 33 c
11 34 c
12 37 c
13 40 c
14 47 c
15 61 c
16 64 c
17 81 c
18 82 c
19 99 c
20 100 c
21 100 c
22 100 c
23 100 c
24 100 c
1 4 a
2 5 a
3 5 a
4 6 a
5 7 a
6 10 a
7 11 a
8 11 a
9 12 a
10 13 a
11 14 a
12 15 a
13 15 a
14 15 a
15 16 a
16 17 a
17 20 a
18 24 a
19 27 a
20 100 a
21 100 a
22 100 a
23 100 a
24 100 a
    };    
\legend{NN,CFL$_r$,CFL$_{iter}$, NC,NA}
\end{axis}
\end{tikzpicture}


==> Figures/Newton+CFL/B1S.tex <==

\begin{tikzpicture}[scale=0.8]
\begin{axis}[
    title = B1S,
    legend pos = north west,
    xlabel={Simulation number},
    ylabel={Required number of iterations}
    ]
    \addplot [
        scatter,
        only marks,
        point meta=explicit symbolic,
        scatter/classes={
            a={mark=*,black},
            b={mark=triangle*,black!50},
            c={mark=triangle*,black!20},
            d={mark=square*,black!50},
            e={mark=square*,black!20}% <-- don't add comma
        },
    ] table [meta=label] {
        x y label
        1 6 d
2 6 d
3 6 d
4 6 d
5 17 d
6 19 d
7 24 d
8 26 d
9 33 d
10 34 d
11 34 d
12 36 d
13 41 d
14 45 d
15 48 d
16 61 d
17 82 d
18 100 d
19 100 d
20 100 d
21 100 d
22 100 d
23 100 d
24 100 d
1 7 e
2 7 e
3 7 e
4 7 e
5 16 e
6 19 e
7 20 e
8 21 e
9 31 e
10 34 e
11 35 e
12 48 e
13 52 e
14 54 e
15 63 e
16 74 e
17 86 e
18 92 e
19 100 e
20 100 e
21 100 e
22 100 e
23 100 e
24 100 e
1 7 b
2 8 b
3 9 b
4 11 b
5 33 b
6 44 b
7 57 b
8 64 b
9 66 b
10 69 b
11 73 b
12 78 b
13 80 b
14 93 b
15 96 b
16 100 b
17 100 b
18 100 b
19 100 b
20 100 b
21 100 b
22 100 b
23 100 b
24 100 b
1 6 c
2 6 c
3 6 c
4 6 c
5 17 c
6 19 c
7 24 c
8 26 c
9 33 c
10 34 c
11 34 c
12 36 c
13 41 c
14 45 c
15 47 c
16 61 c
17 82 c
18 100 c
19 100 c
20 100 c
21 100 c
22 100 c
23 100 c
24 100 c
1 4 a
2 5 a
3 5 a
4 5 a
5 11 a
6 14 a
7 17 a
8 18 a
9 26 a
10 32 a
11 35 a
12 41 a
13 45 a
14 46 a
15 50 a
16 59 a
17 71 a
18 100 a
19 100 a
20 100 a
21 100 a
22 100 a
23 100 a
24 100 a
    };    
\legend{NN,CFL$_r$,CFL$_{iter}$, NC,NA}
\end{axis}
\end{tikzpicture}

==> Mainmatter/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
The neural network presented in this paper was able to predict a local CFL number such that it accelerated the convergence for pseudo time-stepping in most of the considered 2D laminar flow simulations. For back-steps B1 to B4, on which the network was trained on, the network was able to accelerate convergence in most cases for B1 and B3, as shown in table \ref{tab:backstepres2}. Surprisingly, the network was not able to accelerate the convergence for most cases for B2 and B4. So, although the network was trained on also varieties these simulations, it was not able to predict optimal CFL numbers. What is also worth to notice, is the fact that the mirrored and the rotated version of B1 all have different results, while they are essentially the same simulation. Still, also for these cases, the network was able to accelerate the convergence in the majority of the considered simulations. 

To investigate generalizability, Couette cylinder flows as well as back-steps and Couette flows with obstacles are also considered. In general, the network performed better on the Couette flows than the back-steps on which is was trained, with the results given in table \ref{tab:couetteres2}. For the simulations with obstacles, the network was also able to accelerate convergence in most cases. In table \ref{tab:resobst}, we can again see that the network performs better on the simulations of BO than the simulations on which it has been trained. Furthermore, in most cases of the Couette with obstacle the network accelerates the convergence. 

In tables \ref{tab:acc} the acceleration of the network is given. For almost all considered simulations, the network accelerated the convergence, if both the network and one of the default CFL numbers led to convergence. The network especially performed much better at simulations of B3 compared to CFL$_{iter}$ and CFL$_e$, as it led to convergence in all simulations, with a mean acceleration of 6. We can again see that B2 and B4 were the simulations where the network performed worst.

Information about convergence is given in table \ref{tab:conv}, where we can see that in the cases that the network has difficulties to lead to convergence, either CFL$_{iter}$ or CFL$_e$ also faces these problems. There are, however, also cases where the network is able to give a converged solution where the default CFL numbers are not, like B3 and BO. So either the network outperforms the default CFL numbers, or it probably faces the same difficulties regarding convergence as the default CFL numbers. 



